Statistically Meaningful Approximation: a Case Study on Approximating Turing Machines with Transformers

A common lens to theoretically study neural net architectures is to analyze the functions they can approximate. However, constructions from approximation theory may be unrealistic and therefore less meaningful. For example, a common unrealistic trick is to encode target function values using infinite precision. To address these issues, this work proposes a formal definition of statistically meaningful (SM) approximation which requires the approximating network to exhibit good statistical learnability. We study SM approximation for two function classes: boolean circuits and Turing machines. We show that overparameterized feedforward neural nets can SM approximate boolean circuits with sample complexity depending only polynomially on the circuit size, not the size of the network. In addition, we show that transformers can SM approximate Turing machines with computation time bounded by $T$ with sample complexity polynomial in the alphabet size, state space size, and $\log (T)$. We also introduce new tools for analyzing generalization which provide much tighter sample complexities than the typical VC-dimension or norm-based bounds, which may be of independent interest.

==> limitations.tex <==
\section{Limitations and societal impact} \label{sec:limitations}
\noindent{\bf Limitations.} While this work proves upper bounds for statistically meaningful approximation, it is unclear how to prove lower bounds for statistically meaningful approximation. For example, the following question would be nice to study and provide more motivation for the defining this new notion of statistically approximation. Are there function classes  $\mfam$  and $\afam$ such that $\mfam$ can approximate $\afam$ in the classical sense but cannot statistically meaningfully approximate $\afam$? A limitation of our definition is that it's nice for providing upper bounds, but the correct formulation for proving a lower bounded is unclear. For example, one could image proving lower bounds for a specific loss $\bell$, e.g. the results could look something like $\mfam$ cannot statistically meaningfully approximate $\afam$ if we use $\bell$ as the surrogate loss. This isn't entirely satisfactory, because ideally the lower bound is more intrinsic to $\mfam$ and doesn't depend on $\bell$. Thus, the right formulation here is still unclear.

\noindent{\bf Negative societal impact.} We don't anticipate negative societal impacts of our work -- this is a theoretical work on approximation theory, and is several layers removed from empirical applications.

==> rnn_lb.tex <==
\section{All-layer margin lower bound for RNNs}
\newcommand{\polylpoly}{polyL/poly}
\newcommand{\polyl}{polylog}
\newcommand{\advice}{s}
\newcommand{\lang}{\gL}
\newcommand{\lmarg}{\marg^{\textup{layer}}}


For simplicity, we focus on RNNs with ReLU activations, though our bounds can be extended to cover a broader class of RNNs with \textit{computable} activations.\footnote{We say an activation is computable if for all $p \ge 1$, there exists a Turing machine to compute the activation up to $p$ bits of precision in $\poly(p)$ time.} We also assume that the Turing machine input $\inp$ is binary, which can be achieved by using the binary encoding of each symbol in $\symbset$. 

Let $\inp \in \{0, 1\}^{\inpsize}$ denote the intended input to the Turing machine. We consider $T'$-step RNNs parameterized by $\param = (W, \bias, \param_{\textup{cls}})$ for a weight $W \in \R^{\width \times (\inpsize + \width)}$ and bias $\bias \in \R^{\width}$, and classifier $\param_{\textup{cls}} \in \R^{\width}$, where the representation for the $i$-th timestep, $\layer_i$, is computed as follows: $\layer_0(\inp, \param) = \zeros$, and
\begin{align}
	\layer_i(\inp, \param) = \relu\left(W\begin{bmatrix}
		\inp \\
		\layer_{i - 1}(\inp, \param)
	\end{bmatrix} + \bias\right)
\end{align}
The output $\mfrnn_{\width, \inpsize, \Time'}$ is obtained via a linear classifier on the $\Time'$-th output: $\mfrnn_{\width, \inpsize, \Time'}(\inp, \param) = \param_{\textup{cls}}^\top \layer_{\Time'}(\inp, \param)$. We can define the following class of RNN functions:
\begin{align}\label{eq:rnn_fam}
	\mfamrnn_{\width, \inpsize, \alpha, \Time'} \triangleq \{\inp \mapsto \mfrnn_{\width, \inpsize, \Time'}(\inp, \param) : \|\param\|_1 \le \avglone \}
\end{align}

To formally introduce our lower bound for the RNN, it will convenient to consider a slightly modified family of Turing machines with 2 tapes, one read-only for the input, and one output tape which allows writing. It is well-known that a single tape Turing machine can simulate multiple-tape Turing machines in with only a quadratic increase in computation time. Thus, the main benefit of this model is that it allows us to disentangle the read-only space from the write-only space, which is important for formally introducing the lower bound. 

Let $\len(\inp)$ denote the number of bits in the binary string $\inp$. We say that $\tm$ is a~\polyl-space Turing machine if there exists a constant $c$ such that for any input $\inp$, $\tm$ terminates using at most $\log^c(\len(\inp))$ space when run on $\inp$. We will define the following class of languages, or subsets of $\{0, 1\}^*$, which is $\epsilon$-approximately recognizable by~\polyl-space Turing machines using polynomial-size advice strings. 

\begin{definition}\label{def:polylpoly}
Choose arbitrary distributions $\dist_1, \dist_2, \ldots$, where $\dist_t$ is a distribution over $\{0, 1\}^t$. We say that $\lang \subset \{0, 1\}^\star$ is~\polylpoly-recognizable with $\epsilon$ error if for every choice of $\dist_1, \dist_2, \ldots$, there exists a~\polyl-space Turing machine $\tm$ and polynomial-sized binary advice strings $\advice_1, \advice_2, \ldots$ such that for all $i$
	\begin{align}
		\Pr_{\inp \sim \dist_i}(\tm((\inp, \advice_i)) \ne \1(\inp \in \lang)) \le \epsilon
	\end{align}
Furthermore, the advice string $\advice_i$ must be polynomial-sized, that is, there exists a $c$ such that for all $i$, $\len(\advice_i) \le i^c$.
\end{definition}
This is not a commonly-studied class of languages in complexity theory; however, L/poly, the class of languages recognizable by a logarithmic-space Turing machine with a polynomial-sized advice string, is well-studied. The definition above modifies L to polylog and only requires the language to be approximately recognizable by the Turing machine.

We pose the following natural computational hardness assumption, which states that not all languages in P are~\polylpoly-recognizable with $\epsilon$ error, for some $\epsilon$. 

\noindent{\bf Computational hardness assumption.} Let P denote the class of languages $\lang \subset \{0, 1\}^*$ such that there exists a Turing machine satisfying $\tm(\inp) = \1(\inp \in \lang)$ which terminates in $\len(\inp)^c$ time for all inputs $\inp$, where $c$ is some constant. We assume there exists some $\epsilon > 0$ and some $\lang$ in P which is not~\polylpoly-recognizable with $\epsilon$ error.

We note that the question of whether P is contained in L/poly is an open question in complexity theory~\citep{aaronson2008complexity}. This assumption strengthens L to polyL, and allows for some error $\epsilon$ in the Turing machine.

Our lower bound result states that if RNNs can approximate Turing machines such that a certain Lipschitzness-based complexity measure is polynomial in the input size with probability $1 - \epsilon$, then the above assumption is violated. For technical reasons, we need to consider an alternative version of the all-layer margin in~\eqref{eq:all_layer_def}, though we conjecture that a similar statement is likely true for the all-layer margin defined in~\eqref{eq:all_layer_def}. On the other hand, we can use the same alternative complexity measure to prove that transformers can meaningfully approximation Turing machines. 

The alternative all-layer margin-based complexity measure is as follows. Consider a general architecture in a slightly modified setting compared to Section~\ref{sec:correction_function}, where there are layer functions $\func_1, \ldots, \func_{\depth}$ parameterized by $\param_1, \ldots, \param_{\depth}$, where the $i$-th hidden layer is defined by 
\begin{align}
	\begin{split}
	\layer_0(\inp, \param) &= \inp\\
	\layer_i(\inp, \param) &=\func_i((\layer_j(\inp, \param))_{j \in \gJ_i}, \param_i)
	\end{split}\label{eq:layer_all_layer_func}
\end{align}
where $\gJ_i \subseteq \{0, \ldots, i - 1\}$ is a generic set of input indices to $\func_i$. For perturbation vectors $\delta_1, \ldots, \delta_{\depth}$, where the dimensionality of $\delta_i$ matches the output dimensionality of $\func_i$, we can also define the perturbed version of the function as follows:
\begin{align}
	\layer_0(\inp, \param, \delta) &= \inp\\
	\layer_i(\inp, \param, \delta) &= \func_i((\layer_j(\inp, \param, \delta))_{j \in \gJ_i}, \param_i) + \delta_i \max\{\max_{j \in \gJ_i} \|\layer_j(\inp, \param, \delta)\|_2, 1\}
\end{align}
with $\Func(\inp, \param, \delta) = \layer_{\depth}(\inp, \param, \delta)$. With this definition, the layer-based all-layer margin is defined by
\begin{align}
	\lmarg_{\Func}(\param, \inp, y) = 
	\begin{split}
		\max_{\delta} \sqrt{\sum_i \|\delta_i\|_2^2} \\
		\text{such that } (y - 0.5) \cdot \Func(\inp, \param, \delta) \le 0
	\end{split}\label{eq:layer_all_layer_def}
\end{align}

\newcommand{\distf}{D}
We can use~\eqref{eq:layer_all_layer_def} to prove meaningful approximation, analogous to Lemma~\ref{lem:all_layer}. We first need to define the following complexity measure of covering a single layer function, as defined above. 
In the setting above, let $\paramset_i$ denote some set of parameters for the $i$-th layer. For $\param, \hparam \in \paramset_i$, define the distance metric $\distf_{\func_i}(\param, \hparam) \triangleq \min_{\layer_0, \ldots, \layer_{i - 1}} \frac{\|\func_i(\layer_0, \ldots, \layer_{i - 1}, \param) - \func_i(\layer_0, \ldots, \layer_{i - 1}, \hparam)\|_2}{\max \{\max_{j \in \gJ_i}\|\layer_j\|_2, 1\}}$.

We define the following covering number of $\paramset_i$. Consider any finite set $\widehat{\paramset_i}$ which $\varepsilon$-covers $\Param_i$ in the following sense: for all $\param \in \paramset_i$, $\exists \hParam \in \widehat{\paramset_i}$ such that $\distf_{\func_i}(\param, \hparam) \le \varepsilon$. 
We define $\gN_i(\varepsilon, \paramset_i)$ to be the minimum $|\widehat{\paramset_i}|$ such that the above holds.The following condition states that $\gN_i(\varepsilon, \paramset_i)$ scales inverse quadratically with $\varepsilon$:
\begin{condition}\label{cond:eps_cover}
	As above, define $\paramset_i$ to be parameter sets for $\func_i$. For all $i$, there exists a covering complexity $\gC_i$ such that the following holds for all $\varepsilon > 0$:
	\begin{align}
		\log \gN_i(\varepsilon, \paramset_i) \le \left\lfloor \frac{\gC^2_i}{\varepsilon^2} \right\rfloor
	\end{align}
\end{condition}
If the above condition holds for all layers in the function family, then we can guarantee meaningful approximation as follows. 
\begin{lemma}\label{lem:layer_all_layer}
	In the setting above, let $\mf$ be an architecture defined in~\eqref{eq:layer_all_layer_func}, and define $\mfam \triangleq \{x \mapsto \mf(x, (\param_1, \ldots, \param_{\depth})) : \param_i \in \paramset_i\}$. Suppose that parameter sets $\paramset_1, \ldots, \paramset_{\depth}$ satisfy Condition~\ref{cond:eps_cover} with covering complexities $\gC_1, \ldots, \gC_{\depth}$. Fix $\epsilon \ge 0$. Let $\afam$ be a family of $\{0, 1\}$-valued functions such that for all $\apprf \in \afam$, there exists $\param = (\param_1, \ldots, \param_{\depth}) \in \paramset$ such that the following holds:
	\begin{align} \label{eq:layer_all_layer:1}
		\E_{x \sim \dist}[\1(\lmarg_{\Func}(\param, x, \apprf(x) < \thresh))] \le  \epsilon
	\end{align}
	Then $\mfam$ $\left( \tildeO\left(\frac{(\sum_i \gC_i)^2}{\thresh^2 \epsilon^2}\right),  \epsilon\right)$-meaningfully approximates $\afam$ with respect to $\ellzo$. 
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:all_layer}]
	Our proof follows Lemma~\ref{lem:all_layer}, with minor modifications. We define $\bell$ as in Lemma~\ref{lem:all_layer}, except we use $\lmarg_{\Func}$ defined in~\eqref{eq:layer_all_layer_def}. 
	
	The main differences are in checking the Rademacher complexity condition for meaningful approximation. First, fixing $\apprf \in \afam$, define $\gL_{\apprf}$ as in Definition~\ref{def:meaningful_approx}. 
	
	We first observe that following the same argument as Claim A.4 of~\citep{wei2019improved}, $|\lmarg_{\Func}(\param, x, y) - \lmarg_{\Func}(\param', x, y)| \le \sqrt{\sum_i \distf_{\func_i}^2(\param_i, \param'_i)}$ for any $\param, \param'$, $\inp, y$. Let $\gN_{1:\depth}(\varepsilon, \paramset)$ denote the size of the smallest $\widehat{\paramset} = \widehat{\paramset_1} \times \ldots \times \widehat{\paramset_{\depth}}$ such that for all $\param \in \paramset$, $\exists \hparam \in \widehat{\paramset}$ with $\sqrt{\sum_i \distf_{\func_i}^2(\param_i, \widehat{\param_i})} \le \varepsilon$. By Lemma A.5 of~\citep{wei2019improved} and Condition~\ref{cond:eps_cover}, 
	\begin{align}
	 \log	\gN_{1:\depth}(\varepsilon, \paramset) \le \left \lfloor \frac{(\sum_i \gC_i)^2}{\varepsilon^2} \right \rfloor
	\end{align}  
	Thus, we can conclude that $\log \gN_{\|\cdot\|_{\infty}}(\varepsilon, \gL_{\apprf}) \le \log \gN_{1:\depth}(\varepsilon, \paramset) \le \left \lfloor \frac{(\sum_i \gC_i)^2}{\varepsilon^2} \right \rfloor$. The remaining steps follow as in Lemma~\ref{lem:all_layer}.
\end{proof}

The following bound applies Lemma~\ref{lem:layer_all_layer} to show that RNNs can meaningfully approximate a generic function family, as long as it can fit the functions with large margin defined in~\eqref{eq:layer_all_layer_def}. The method for applying the bound essentially unrolls the RNN and views it as a deep feedforward network with untied parameters between layers. 
\begin{lemma}
	In the RNN setting, let $\mfamrnn_{\width, \inpsize, \avglone, \Time'}$ be defined as in~\eqref{eq:rnn_fam}. We can view an RNN in the form described in~\eqref{eq:layer_all_layer_func} by setting $\depth = \Time' + 2$ and $\func_1 = \zeros$, $\func_i(\cdot, \cdot, (W, \bias)) = x, \layer \mapsto \relu\left(W \begin{bmatrix}
		x\\
		\layer
	\end{bmatrix} + \bias\right)$ and $\gJ_i = \{0, i - 1\}$ for $2 \le i \le \depth - 1$. We also set
	with $\func_{\depth}(\cdot, \param_{\textup{cls}}) = \layer \mapsto  \param_{\textup{cls}}^\top \layer$. Let $\afam$ be a family of $\{0, 1\}$-valued functions such that for all $\apprf \in \afam$, there exists $\param$ with $\|\param\|_1 \le \avglone$ where the following holds:
	\begin{align}
		\E_{\inp \sim \dist}[\1(\lmarg_{\mfrnn_{\width, \inpsize, \Time'}}(\param, \inp, \apprf(\inp)) < \thresh)] \le \epsilon
	\end{align}
	Then $\mfamrnn_{\width, \inpsize, \avglone, \Time'}$ $\left(\tilde{O}\left(\frac{B^2}{\epsilon^2}\right), \epsilon\right)$-meaningfully approximates $\afam$ w.r.t $\ellzo$. Here $B^2 = \frac{\avglone^2 (\Time')^2\log(\width)}{\thresh^2}$ is referred to as the complexity of the approximation.
\end{lemma}
\begin{proof}
	Note that this formulation unrolls the RNN and essentially views each timestep as using a distinct set of parameters. Thus, it suffices to bound $\log \gN_i (\epsilon, \paramset_i)$ where $\paramset_i = \{(W, b) : \|W\|_1 + \|b\|_1 \le \avglone\}$, for $i < \depth$, and $\log \gN_{\depth}(\epsilon, \paramset_{\depth})$, where $\paramset_{\depth} = \{\param_{\textup{cls}} : \|\param_{\textup{cls}}\|_1 \le \avglone\}$. Note that for both of these, standard arguments for bounding the covering number of $\|\cdot\|_1$-norm bounded parameter sets apply (see Section B of~\citep{wei2019improved}). (We also need to reason about the worst-case Lipschitzness of the ReLU activation $\relu$; standard arguments apply here.)
\end{proof}
We can now rigorously state our result contrasting RNNs and transformers for approximating Turing machines. We consider the following class of Turing machines:

\begin{theorem}\label{thm:rnn_lb}
	In the setting above, consider the following class of Turing machines:
	\begin{align}
		\afam \triangleq \{x \mapsto \1(x \in \lang) : \lang \textup{ is in P}\} 
	\end{align}
 Suppose that for every $\apprf \in \afam$, all $\inpsize$, all choices of distributions $\dist_{\inpsize}$ over $\{0, 1\}^{\inpsize}$, and any $\epsilon > 0$, there exists an RNN $ \mfrnn_{\width(\inpsize), \inpsize, \Time'(\inpsize)}(\cdot, \param)$ such that $\Time'(\inpsize) \le \exp(\poly(\inpsize))$, $\width(\inpsize) \le \textup{polylog}(\inpsize)$, and $\|\param\|_1 \le \exp(\poly(\inpsize))$, and 
	\begin{align}\label{eq:rnn_lb:1}
		\E_{\dist_i}\left[\1\left(\lmarg_{\mfrnn_{\width(\inpsize), \inpsize, \Time'(\inpsize)}}(\param, \inp, \apprf(\inp)) < \frac{c_1 \Time'(\inpsize)\|\param\|_1}{\inpsize^{c_2}}\right)\right] \le \epsilon 
	\end{align}
	for any constant $c_1, c_2$. Then the computational hardness assumption above is violated. In other words, if the computational hardness assumption holds, then RNNs with~\polyl-width, exponential time horizon, and exponential parameter norm in the input size $i$ must have the quantity $B$ in Lemma~\ref{lem:layer_all_layer} be superpolynomially large in $\inpsize$. Thus, the all-layer margin defined in~\eqref{eq:layer_all_layer_def} and bound in Lemma~\ref{lem:layer_all_layer} cannot be used to show meaningful approximation with complexity polynomial in the input size.
\end{theorem}

Our proof will rely on leveraging the all-layer margin bound to simulate the RNN with low precision. For any real number $v$, let $\bin_i(v)$ denote the coefficient of $2^i$ in the binary representation of $|v|$. We say that a real number $v \in \R$ has $p$ bits of relative precision if $\max \{i : \bin_i(v) = 1\} - \min\{i : \bin_i(v) = 1\} \le p$. We say that a vector (or matrix) $v$ has $p$ bits of relative precision if all of its entries have $p$ bits of relative precision. We note that if $v$ has $p$ bits of relative precision, then it can be represented with $p + \lceil\log(|\max\{i : \bin_i(v) = 1\}|)\rceil + 1 = O(p + \log |\log (v)|)$ bits, by storing a binary representation of $\max\{i : \bin_i(v) = 1\}$ as well as the $p$ bits of $v$. We say that $v$ has $p$ bits of absolute precision if $\min\{i : \bin_i(v) = 1\} \ge -p$.


\begin{lemma}\label{lem:trunc_precision}
	In the setting of Theorem~\ref{thm:rnn_lb}, let $f(\cdot, \cdot, (W, \bias)) \triangleq x, \layer \mapsto \relu\left(W \begin{bmatrix}
		x\\
		\layer
	\end{bmatrix} + \bias\right)$ denote the function computing a single timestep of the RNN. Suppose that for $\param = (W, \bias, \param_{\textup{cls}})$,
	\begin{align}\label{eq:trunc_precision:1}
		\lmarg_{\mfamrnn_{\width, \inpsize, \Time'}}(\param, \inp, y) \ge \frac{\Time'(\inpsize) \|\param\|_1}{r}
	\end{align}
	Then consider any $\hlayer_0, \hlayer_1, \ldots, \hlayer_{\Time'}$, where $\hlayer_i$ has $O(\log r)$ bits of absolute and relative precision and satisfies
	\begin{align}
		\hlayer_0  = \layer_0 &= \zeros_{\width}\\
		\|\hlayer_i -  \func(\inp, \hlayer_{i - 1}, (W, \bias))\|_2 &\le \frac{\max\{\|\func(\inp, \hlayer_{i - 1}, (W, \bias))\|_2, 1\}}{3r}
	\end{align}
	It must hold that $|\param_{\textup{cls}}^\top \hlayer_{\Time'}| \ge \frac{1}{r}$.
\end{lemma}
\begin{proof}
	We will construct a perturbation $\delta = (\delta_1, \ldots, \delta_{\Time' + 1})$ as follows. Define 
	\begin{align}
		\delta_i \triangleq \frac{(\hlayer_i - \func(\inp, \hlayer_{i - 1}, (W, \bias)))}{\max\{\|\inp\|_2, 1, \hlayer_{i - 1}\}}
	\end{align}
	Note that 
	\begin{align}
		\|	\delta_i \|_2 &= \frac{1}{\max\{\|\inp\|_2, 1, \hlayer_{i - 1}\}} \|\hlayer_i -  \func(\inp, \hlayer_{i - 1}, (W, \bias))\|_2\\
		&\le \frac{\|\func(\inp, \hlayer_{i - 1}, (W, \bias))\|_2}{3r\max\{\|\inp\|_2, 1, \hlayer_{i - 1}\}}\\
		&< \frac{(\|W\|_1 + \|\bias\|_1)(\|\inp\|_2 + 1 + \|\hlayer_{i - 1}\|_2)}{3r\max\{\|\inp\|_2, 1, \hlayer_{i - 1}\}} \tag{based on Lipschitzness of $\relu$}\\
		&< \frac{\|W\|_1 + \|\bias\|_1}{r}
	\end{align}
	Note that we used a very rough bound in the third inequality. First, consider the case where $\delta_{\Time'} = 0$. 
	Then we note that 
	\begin{align}
	\sqrt{	\sum_{i = 1}^{\Time' + 1} \|\delta_i\|_2^2} \le \sqrt{\Time'} \frac{\|W\|_1 + \|\bias\|_1}{r} 
	\end{align}
	Furthermore by construction of $\delta$, we observe that $\mfrnn_{\width, \inpsize, \Time'}(\inp, \param, \delta) = \param_{\textup{cls}}^\top \hlayer_{\Time'}$. 
	Therefore, by the definition of all-layer margin, it must hold that 
	\begin{align}
		\sign(\param_{\textup{cls}}^\top \hlayer_{\Time'}) = \sign(\mfrnn_{\width, \inpsize, \Time'}(\inp, \param, \delta)) = \sign(y - 0.5)
	\end{align}
	On the other hand, now consider the case where $\delta_{\Time' + 1} = -\frac{\param_{\textup{cls}}^\top \hlayer_{\Time'}}{\max\{1, \|\hlayer_{i - 1}\|_2\}}$. Since this perturbation does change the label for $\mfrnn_{\width, \inpsize, \Time'}(\inp ,\param, \delta)$, we must have 
	\begin{align}
		\frac{|\param_{\textup{cls}}^\top \hlayer_{\Time'}|}{\max\{1, \|\hlayer_{i - 1}\|_2\}} + \sqrt{\Time'} \frac{\|W\|_1 + \|\bias\|_1}{r}  \ge \sqrt{\sum_{i = 1}^{\Time' + 1} \|\delta_i\|_2^2}
		> \lmarg_{\mfamrnn_{\width, \inpsize, \Time'}}(\param, \inp, y)
	\end{align}
	Thus, plugging in~\eqref{eq:trunc_precision:1}, we must have 
	\begin{align}
		\frac{|\param_{\textup{cls}}^\top \hlayer_{\Time'}|}{\max\{1, \|\hlayer_{i - 1}\|_2\}} \gtrsim \frac{\|\param_{\textup{cls}}\|_1}{r}
	\end{align}
	Thus, rearranging and using $\|\param_{\textup{cls}}\|_2 \le \|\param_{\textup{cls}}\|_1$, it follows that 
	\begin{align}
		\frac{\param_{\textup{cls}}^\top}{\|\param_{\textup{cls}}\|_2}\hlayer_{\Time'} \gtrsim \frac{1}{r}
	\end{align}
	From the approximating RNN which satisfies~\eqref{eq:rnn_lb:1}, we construct a~\polyl-space Turing machine and polynomial-sized advice strings for recognizing the language. 
\end{proof}
In contrast, we show that the margin defined in~\eqref{eq:layer_all_layer_def} can be used to show that transformers meaningfully approximate Turing machines with complexity polynomial in the input size. 

\begin{theorem}\label{thm:turing_approx_comparison}
	In the setting above, consider the class \begin{align}
		\afam_{\numstates} \triangleq \{x \mapsto \1(x \in \lang) : \lang \textup{ in P, computed by Turing machine with } \le \numstates \textup{ states, } \len(x)^c \textup{ time }\}
	\end{align} of functions computed by polynomial-time Turing machines with at most $\numstates$ states and $\inpsize^c$ time, where $\inpsize$ is the input size and $c$ is some constant. Fix any $\inpsize$ and choose transformer width $\width \gtrsim \numstates + c \log(\inpsize)$, depth $\depth \gtrsim c\log(\inpsize)$, $\|\cdot\|_1$-norm bound $\avglone \ge \poly(\numstates, \depth)$, and $\Time' = \inpsize^c$ steps. Then for $\apprf \in \afam_{\numstates}$, $\exists \param$ with $\|\param\|_1 \le \avglone$ such that for all $\inp \in \{0, 1\}^{\inpsize}$,
\begin{align}
	\lmarg_{\mftr_{\width, \depth, \Time'}}(\param, \inp, \apprf(\inp)) \ge \frac{1}{\poly(\numstates, c \log(\inpsize))}
\end{align} 
As a consequence, the margin $\lmarg$ defined in~\eqref{eq:layer_all_layer_def} and Lemma~\ref{lem:layer_all_layer} can be used to show that for any distribution $\dist_{\inpsize}$ over $\{0, 1\}^{\inpsize}$, $\mfamtr_{\width, \depth, \avglone, \Time}$ $\left(\poly(\avglone) \tildeO\left(\frac{\inpsize^{2c} \log (\width \depth)}{\epsilon^2}\right), \epsilon\right)$-meaningfully approximates $\afam_{\numstates}$ with respect to $\ellzo$. 
\end{theorem}
As the proof follows the same steps as Theorem~\ref{thm:turing_approx}, we only provide a sketch here. 
\begin{proof}[Proof sketch of Theorem~\ref{thm:turing_approx_comparison}]
	We follow the same proof sketch as Theorem~\ref{thm:turing_approx}. We use the exact same Turing machine construction, and instead of proving Theorem~\ref{thm:abstract} for the margin defined in~\eqref{eq:all_layer_def}, we prove a variant for the one defined in~\eqref{eq:layer_all_layer_def}. The proof follows with the same steps and conditions. The difference is that~\eqref{eq:layer_all_layer_def} doesn't allow for parameter sharing, so we treat each of the transformer parameters as distinct ones for each timestep. This results in the extra $(\Time')^2 = \inpsize^{2c}$ factor in the complexity bound.
\end{proof}

